Topic-wise Exploration of the Telegram Group-verse

Although Telegram is currently one of the most popular instant messaging apps in the world, previous studies have mainly focused on analysing discussions on specific angles and topics. In this paper, we present a broad analysis of publicly accessible groups that cover a wide range of discussions, including Education, Erotic, Politics, and Cryptocurrencies. How do people interact with different topic groups? Is there any common or peculiar behaviour? We engineer and offer an open-source tool to automate the collection of messages from Telegram groups, a non-straightforward problem. We use it to collect more than 51 million messages from 669 groups. Here, we present a first-of-its-kind, per-topic analysis, contrasting the users' activity patterns from different angles -- the language, the presence of bots, the type and volume of shared media content, links to external platforms, etc. Our results confirm some anecdotal evidence, e.g., indications of spamming behaviour, and unveil some unexpected findings, e.g., the different sharing patterns of video and message length in groups of different topics. Our research provides a horizontal analysis of the public group in Telegram across various general topics, establishing a foundation for future studies that can delve deeper into user interactions and content dynamics within this unique messaging environment.

==> makefile <==
DOC=main

all:
	pdflatex $(DOC)
	bibtex   $(DOC)
	pdflatex $(DOC)
	pdflatex $(DOC)

clean:
	find . -name '*~' -exec rm -f {} \;
	find . -name '*.aux' -exec rm -f {} \;
	rm diff.* \;
	rm -f texput.log $(DOC).log $(DOC).ps $(DOC).toc $(DOC).lo* $(DOC).bbl $(DOC).blg $(DOC).dvi $(DOC).out $(DOC).synctex.gz
	
zip: ${sources} ${pdffiles}
	rm -f $(DOC).zip && zip -r $(DOC).zip *.tex *.bib *.bbl *.cls figures Makefile makefile
	
diff:
		latexdiff  -c submission-version/latexdiff_conf.txt --preamble=submission-version/latexdiff_preamble.tex \
	              --flatten submission-version/$(DOC).tex $(DOC).tex > diff.tex
		cat diff.tex | sed 's/\\DIFaddbegin \\bibitem/\\bibitem/g' | sed 's/]\\DIFaddend/]/g' | sed -e '/{\\DIFaddbegin \\DIFadd{/ s/}}/}/g' | sed 's/{\\DIFaddbegin \\DIFadd{/{/g' > /tmp/diff.tex
		cp /tmp/diff.tex diff.tex
		rm -f diff.aux
		pdflatex diff
		pdflatex diff


==> text/2-related_discarded.tex <==
\section{Related work TO DISCARD}


Several studies have delved into the characteristics and dynamics of messaging platforms such as Telegram. Dargahi Nobari \textit{et al.} (2021)~\cite{dargahi_nobari_characteristics_2021} examined the hybrid nature of Telegram, serving both public and private communication needs. Baumgartner \textit{et al.} (2020)~\cite{baumgartner_pushshift_2020} emphasized the platform significance in studying online social movements, extremism, and disinformation, presenting a valuable dataset for such analysis. Hashemi and Zare Chahooki (2019)~\cite{hashemi_telegram_2019} provided insights into the behavior of Iranian users on Telegram, underscoring its popularity and unique features.

% Analyzing Content and Communities:
To delve into the workings of messaging platforms like Telegram, researchers have focused on dissecting the structural and topical elements of messages. Dargahi Nobari \textit{et al.} (2017) \cite{dargahi_nobari_analysis_2017} undertook such analysis by examining these aspects within Telegram messages. Tikhomirova and Makarov (2021) \cite{tikhomirova_community_2021} expanded on this by specifically investigating the detection of communities within Telegram channels, exploring different models for this task. Additionally, Maros \textit{et al.} (2020) \cite{maros_analyzing_2020} delved into the usage of audio messages within WhatsApp groups, studying the properties of content and how it spreads.

%Security
Advancements in digital security often hinge on the analysis of emerging threats and vulnerabilities. Morgia et al. (2023) \cite{morgia_its_2023}  conducted a large-scale analysis to identify and analyze fake channels on Telegram, proposing a machine-learning model for detection. Satrya et al. (2016) \cite{satrya_digital_2016} detailed artifacts generated by Telegram Messenger on Android, facilitating digital forensic investigation while Anglano et al. (2017) \cite{anglano_forensic_2017} introduced a methodology aiding in the comprehensive reconstruction of user activities. 
% Social Impacts and Extremism:
Akbari and Gabdulhakov (2019) \cite{akbari_platform_2019} analyzed challenges faced by Telegram in Iran and Russia, focusing on government surveillance and resistance movements. 
Khawaja (2017) \cite{khawaja_telegram_2017} highlighted the use of Telegram by terrorist organizations like ISIS, emphasizing its role in propaganda dissemination and recruitment.

Several studies have focused on examining group content to identify indicators of manipulation, coordination for illicit activities, or dissemination of hate speech. Weerasinghe et al. (2020) \cite{weerasinghe_pod_2020} explored the manipulation of social media popularity through reciprocity abuse in Telegram-hosted pods. Agarwal et al. (2022)  \cite{agarwal_jettisoning_2022} addressed the issue of unwanted junk messaging on WhatsApp, proposing machine learning models for detection. Xu et al. (2019)\cite{xu_anatomy_2019} conducted an empirical study of pump-and-dump activities in cryptocurrency markets, presenting a model for fraud detection.
Naseri and Zamani (2019) \cite{naseri_analyzing_2019} studied news popularity analysis and prediction in Telegram, contrasting its features with traditional social media platforms. Saha et al. (2021) \cite{saha_short_2021} investigated fear speech in Indian WhatsApp groups, considering its impact on inter-group conflict. Wich et al. (2022) \cite{wich_introducing_2022} developed an abusive language classification framework for Telegram messages in German, addressing the spread of hate speech. 


Hashemi and Zare Chahooki (2019) \cite{hashemi_telegram_2019} measured group quality in Telegram, identifying features indicative of high-quality groups. Nikkhah et al. (2018) \cite{nikkhah_telegram_2018} examined the use of Telegram by Iranian immigrants, focusing on communication tools and online communities throughout the immigration process. Maros et al. (2020) \cite{maros_analyzing_2020} explored the use of audio messages in WhatsApp groups, characterizing content properties and their impact.

% Comparative Studies:
% Sutikno et al. (2016) compared WhatsApp, Viber, and Telegram, analyzing their features and user preferences.
